Analysis of DAWNBench, a Time-to-Accuracy Machine Learning Performance Benchmark

Researchers have proposed hardware, software, and algorithmic optimizations to improve the computational performance of deep learning. While some of these optimizations perform the same operations faster (e.g., increasing GPU clock speed), many others modify the semantics of the training procedure (e.g., reduced precision), and can impact the final model's accuracy on unseen data. Due to a lack of standard evaluation criteria that considers these trade-offs, it is difficult to directly compare these optimizations. To address this problem, we recently introduced DAWNBench, a benchmark competition focused on end-to-end training time to achieve near-state-of-the-art accuracy on an unseen dataset---a combined metric called time-to-accuracy (TTA). In this work, we analyze the entries from DAWNBench, which received optimized submissions from multiple industrial groups, to investigate the behavior of TTA as a metric as well as trends in the best-performing entries. We show that TTA has a low coefficient of variation and that models optimized for TTA generalize nearly as well as those trained using standard methods. Additionally, even though DAWNBench entries were able to train ImageNet models in under 3 minutes, we find they still underutilize hardware capabilities such as Tensor Cores. Furthermore, we find that distributed entries can spend more than half of their time on communication. We show similar findings with entries to the MLPERF v0.5 benchmark.

==> factor_analysis.tex <==
\subsection{Factor Analysis}
\label{sec:factor_analysis}

In this section, we perform a factor analysis on the optimizations for the
winning entry for CIFAR10 on publicly available hardware. Using a custom
wide ResNet~\cite{zagoruyko2016wide} with mixed-precision
training~\cite{micikevicius2017mixed}, large minibatch
training~\cite{dean2012large}, and cyclic learning rates~\cite{smith2017super} the model trained to 94\% top-1 accuracy on CIFAR10 with a NVIDIA V100 GPU in 6 minutes and 45 seconds for \$0.26.
Applying all these optimizations in conjunction gives a 3.14$\times$ speedup
in time-to-94\% accuracy as shown in Figure~\ref{fig:cifar10-factor-analysis}.
In addition, turning off each of these optimizations individually gives as much
as a 2.91$\times$ slowdown.

\begin{figure*}[t!]
  \centering
  \begin{subfigure}{.6\columnwidth}
    \includegraphics[width=0.99\columnwidth]{figures/cifar10_lesion_factor_analysis_part1.pdf}
    \vspace{-0.5em}
    \caption{Factor analysis}
  \end{subfigure}
  \begin{subfigure}{.6\columnwidth}
    \includegraphics[width=0.99\columnwidth]{figures/cifar10_lesion_factor_analysis_part2.pdf}
    \vspace{-0.5em}
    \caption{Lesion study}
  \end{subfigure}
  \vspace{-0.5em}
  \caption{
    Lesion study and factor analysis for the one V100 Wide ResNet-32 CIFAR10
    entry. We cumulatively added optimizations on at a time for the factor
    analysis. We individually removed optimizations for the lesion study. All
    optimizations give significant speedups, indicating the co-evolution of
    statistical and hardware improvements can dramatically improve performance.
    The baseline ran the Wide ResNet-32 on a P100.
  }
  \label{fig:cifar10-factor-analysis}
  \vspace{-0.5em}
\end{figure*}



==> optimzations.tex <==
\section{Impact of Optimizations}
\label{sec:entry-analysis}

In this section, we analyze the top \dawnbench entries for image classification
to better understand the impact of the various optimizations used.
First, we report general trends in the submissions, showing that hardware,
software, and statistical optimizations are necessary for high performance.
Then, we perform a factor analysis and lesion study on a CIFAR10 entry to
demonstrate the range of optimizations used to speed up deep learning workloads.

\subsection{Overall Trends}

To better understand the speedups seen in the \dawnbench entries, we plot the
time to achieve the required accuracy for CIFAR10 and ImageNet in
Figure~\ref{fig:epoch-time-vs-total-time}. While many optimizations improved the
time per epoch, several also reduced the number of epochs needed for
convergence. We discuss some optimizations in more detail below.

\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.75\textwidth]{figures/e2e_time_vs_hardware_efficiency.pdf}
  \caption{
    Time per epoch vs. the total time to achieve accuracy target for ImageNet
    (left) and CIFAR10 (right) entries. Most entries use software and hardware optimizations to
    reach the accuracy threshold faster and some use statistical optimizations to converge faster.
  }
  \label{fig:epoch-time-vs-total-time}
  % \vspace{-1em}
\end{figure*}


%\minihead{Software Optimizations}
%Properly configuring and using hardware resources made a significant difference
%to performance. Simply changing the TensorFlow version from 1.7 to 1.8
%gives a 1.4$\times$ decrease in training time for AmoebaNet.
%In addition, most entries use optimized communication libraries (NCCLv2) and
%efficient image loading libraries (\texttt{libjpeg-turbo}, \texttt{Pillow-SIMD})
%to give significant performance improvements.
% (TODO: quantify this?). do for camera ready

\minihead{Statistical Optimizations}
Optimizations like progressive image resizing~\cite{lim2017enhanced,
karras2017progressive} and cyclical learning rates~\cite{smith2017super} also
dramatically helped improve performance by reducing the total number of epochs
needed to reach the accuracy threshold. For example, on ImageNet, a standard
ResNet-50 on TPUs took 87 epochs to converge, while a ResNet-50 with progressive
resizing on V100s took 41 epochs to converge. Thus, simple statistical
optimizations can result in over 2$\times$ improvement in statistical
efficiency.

\begin{figure*}[t!]
  \centering
  \includegraphics[width=1.55\columnwidth]{figures/time_vs_cost.pdf}
  \caption{
    Time vs. cost for the various entries submitted to \dawnbench, grouped by
    the device used. We show a zoomed-in version of the box in the plot on the left on the
    right. Different hardware substrates have different pareto frontiers. The
    costs of all entries that use TPU Pods were extrapolated using the cost of
    a single TPU in the cloud.
  }
  \label{fig:time-vs-cost}
  % \vspace{-1em}
\end{figure*}

\minihead{Trade-offs between Time and Cost}
Most of the \dawnbench entries were run on the public cloud, and it was easy to
compute the cost of training a model to the desired accuracy level.
Figure~\ref{fig:time-vs-cost} shows the time versus cost for the different
entries. We observe different pareto frontiers between cost and time for the
different device types, e.g., CPUs are expensive compared to TPUs and GPUs.
TPU Pods are not publicly available, but we
extrapolated their cost in the cloud by multiplying the price of a single TPU by
the number of TPUs used.

Some entries are pareto optimal to others, e.g., the right-most TPU entry
is more expensive and takes longer than the TPU entry just to the left of it.
These are by-products of optimizations (e.g., improvements in TensorFlow and
a different model architecture that converges to the target accuracy in
fewer epochs) applied while keeping the hardware
configuration the same, resulting in entries that achieve the accuracy target
faster at the same cost-per-unit-time.


